Automated Dynamic Mechanism Design

We study Bayesian automated mechanism design in unstructured dynamic environments, where a principal repeatedly interacts with an agent, and takes actions based on the strategic agent's report of the current state of the world. Both the principal and the agent can have arbitrary and potentially different valuations for the actions taken, possibly also depending on the actual state of the world. Moreover, at any time, the state of the world may evolve arbitrarily depending on the action taken by the principal. The goal is to compute an optimal mechanism which maximizes the principal's utility in the face of the self-interested strategic agent. We give an efficient algorithm for computing optimal mechanisms, with or without payments, under different individual-rationality constraints, when the time horizon is constant. Our algorithm is based on a sophisticated linear program formulation, which can be customized in various ways to accommodate richer constraints. For environments with large time horizons, we show that the principal's optimal utility is hard to approximate within a certain constant factor, complementing our algorithmic result. We further consider a special case of the problem where the agent is myopic, and give a refined efficient algorithm whose time complexity scales linearly in the time horizon. Moreover, we show that memoryless mechanisms do not provide a good solution for our problem, in terms of both optimality and computational tractability. These results paint a relatively complete picture for automated dynamic mechanism design in unstructured environments. Finally, we present experimental results where our algorithms are applied to synthetic dynamic environments with different characteristics, which not only serve as a proof of concept for our algorithms, but also exhibit intriguing phenomena in dynamic mechanism design.

==> Automated Dynamic Mechanism Design, arxiv/app.tex <==
\section{Omitted Proofs from Section~\ref{sec:general}}

\begin{proof}[Proof of Theorem~\ref{thm:long}]
    We consider the case where payments are not allowed, i.e., $p_t(h, s) = 0$ for all $h \in \cH$ and $s \in \cS$.
    The case with payments and dynamic IR constraints is essentially the same.
    We use a similar reduction from MAX-SAT to the ones in \cite{papadimitriou1987complexity,mundhenk2000complexity} for partially observable Markov decision processes (POMDPs).
    Given a MAX-SAT instance with $n$ variables $x_1, \dots, x_n$ and $m$ clauses $c_1, \dots, c_m$ where $c_i = \{\ell_{i, j}\}_{j \in [k_i]}$ and each $\ell_{i, j}$ is a literal, we construct a dynamic environment where $T = n$, $|\cS| = m + 1$, and $|\cA| = 2$.
    The goal is to show that the maximum utility is precisely the fraction of clauses that can be simultaneously satisfied.
    Without loss of generality, we assume that no clause contains both the positive literal and the negative literal of a same variable.
    We first describe $\cS$ and $\cA$.
    Each clause $c_i$ corresponds to a unique state in $\cS$, $s_i$.
    In addition to these $m$ states, there is another state $s_0$.
    $\cA$ consists of two actions: $a_\mathrm{pos}$ and $a_\mathrm{neg}$.
    The transition operator and the principal's valuation function are such that:
    \begin{itemize}
        \item The initial distribution is uniform over $\{s_i\}_{i \in [m]}$, i.e., $\trans_0(s_i) = 1 / m$ for each $i \in [m]$.
        \item For each $t \in [T]$ and $a \in \cA$,
        \[
            \trans_t(s_0, a, s_0) = 1 \quad \text{and} \quad \vp_t(s_0, a) = 0.
        \]
        Moreover, for each $t \in [T]$ and $i \in [m]$:
        \begin{itemize}
            \item If $x_t^+ \in c_i$, then
            \[
                \trans_t(s_i, a_\mathrm{pos}, s_0) = \trans_t(s_i, a_\mathrm{neg}, s_i) = 1,
            \]
            and
            \[
                \vp_t(s_i, a_\mathrm{pos}) = 1 \quad \text{and} \quad \vp_t(s_i, a_\mathrm{neg}) = 0.
            \]
            \item if $x_t^- \in c_i$, then
            \[
                \trans_t(s_i, a_\mathrm{pos}, s_i) = \trans_t(s_i, a_\mathrm{neg}, s_0) = 1,
            \]
            and
            \[
                \vp_t(s_i, a_\mathrm{pos}) = 0 \quad \text{and} \quad \vp_t(s_i, a_\mathrm{neg}) = 1.
            \]
            \item otherwise,
            \[
                \trans_t(s_i, a_\mathrm{pos}, s_i) = \trans_t(s_i, a_\mathrm{neg}, s_i) = 1,
            \]
            and
            \[
                \vp_t(s_i, a_\mathrm{pos}) = \vp_t(s_i, a_\mathrm{neg}) = 0.
            \]
        \end{itemize}
        \item The principal and the agent are in a zero-sum situation, i.e., for any $t \in [T]$, $s \in \cS$, $a \in \cA$,
        \[
            \va_t(s, a) = 1 - \vp_t(s, a).
        \]
    \end{itemize}

    Now we show that the maximum utility is precisely the fraction of clauses that can be simultaneously satisfied.
    First observe that without loss of generality, an optimal mechanism depends only on time (and not on the reported states).
    This is because of the zero-sum situation: if the mechanism depends on the reports, then the agent can always choose the worst sequence of actions, which can only make the principal's utility smaller.
    Moreover, given the above observation, without loss of generality, an optimal mechanism is deterministic.
    This is because the overall utility of the principal is linear in the action at any time $t$, so one can always round a randomized mechanism into a deterministic one with at least the same overall utility.
    
    Given the above observations, an optimal mechanism corresponds precisely to a way of assigning values to variables in the MAX-SAT instance: for each $t \in [T]$, the action at time $t$ is $a_\mathrm{pos}$ iff the variable $x_t = 1$ (i.e., the literal $x_t^+$ is chosen).
    Moreover, when the initial state is $s_i$, the onward utility is $1$ if the clause $c_i$ is satisfied by the above assignment, and $0$ otherwise.
    Since the initial state is uniformly at random among $\{s_i\}_{i \in [m]}$, the maximum utility is precisely the maximum fraction of clauses that are satisfiable by some assignment.
    The theorem then follows from the fact that MAX-SAT is hard to approximate within a factor of $7/8 + \eps$ for any $\eps > 0$ \cite{haastad2001some}.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:obj}]
    For brevity, let $\mathrm{obj}$ denote the objective, i.e.,
    \[
        \mathrm{obj} = \sum_{h \in \cH, s \in \cS: (h, s)\text{ is feasible}} \left(\sum_{a \in \cA} \vp_{|h| + 1}(s, a) \cdot x(h, s, a) + y(h, s)\right).
    \]
    Moreover, for each $h \in \cH$, $s \in \cS$, let
    \[
        \mathrm{obj}(h, s) = \sum_{h' \in \cH, s' \in \cS: (h, s) \subseteq (h', s')} \left(\sum_{a \in \cA} \vp_{|h'| + 1}(s', a) \cdot x(h', s', a) + y(h', s')\right).
    \]
    Observe that
    \[
        \mathrm{obj} = \sum_{s \in \cS} \mathrm{obj}(\emptyset, s).
    \]

    We first prove inductively that for each $h \in \cH$, $s \in \cS$,
    \[
        \mathrm{obj}(h, s) = z(h, s) \cdot \up^M(h, s).
    \]
    When $|h| = T - 1$, by the definition of feasible extensions and the construction of the mechanism,
    \begin{align*}
        \mathrm{obj}(h, s) & = \sum_{a \in \cA} \vp_T(s, a) \cdot x(h, s, a) + y(h, s) \\
        & = z(h, s) \cdot \left(\sum_{a \in \cA} \vp_T(s, a) \cdot \pi(h, s, a) + p(h, s) \right) \\
        & = z(h, s) \cdot \up^M(h, s).
    \end{align*}
    When $|h| < T - 1$, for similar reasons,
    \begin{align*}
        \mathrm{obj}(h, s) & = \sum_{h', s': (h, s) \subseteq (h', s')} \left(\sum_{a \in \cA} \vp_{|h'| + 1}(s', a) \cdot x(h', s', a) + y(h', s')\right) \\
        & = \sum_{a \in \cA} \vp_{|h| + 1}(s, a) \cdot x(h, s, a) + y(h, s) \\
        & \phantom{\ =\ } + \sum_{h', s': (h, s) \subseteq (h', s'), |h'| > |h|} \left(\sum_{a \in \cA} \vp_{|h'| + 1}(s', a) \cdot x(h', s', a) + y(h', s')\right) \\
        & = z(h, s) \cdot \left(\sum_{a \in \cA} \vp_{|h| + 1}(s, a) \cdot \pi(h, s, a) + p(h, s)\right) \\
        & \phantom{\ =\ } + \sum_{a', s'': \trans_{|h| + 1}(s, a', s'') > 0} \sum_{h', s': (h + (s, a'), s'') \subseteq (h', s')} \left(\sum_{a \in \cA} \vp_{|h'| + 1}(s', a) \cdot x(h', s', a) + y(h', s')\right)
    \end{align*}
    By the induction hypothesis, the second sum above is equal to
    \begin{align*}
        & \phantom{\ =\ } \sum_{a', s'': \trans_{|h| + 1}(s, a', s'') > 0} \mathrm{obj}(h + (s, a'), s'') \\
        & = \sum_{a', s'': \trans_{|h| + 1}(s, a', s'') > 0} z(h + (s, a'), s'') \cdot \up^M(h + (s, a'), s'') \\
        & = \sum_{a', s'': \trans_{|h| + 1}(s, a', s'') > 0} x(h, s, a') \cdot \etrans_{|h| + 1}(s, a', s'') \cdot \up^M(h + (s, a'), s'') \\
        & = \sum_{a \in \cA, s' \in \cS} x(h, s, a) \cdot \trans_{|h| + 1}(s, a, s') \cdot \up^M(h + (s, a), s') \\
        & = z(h, s) \cdot \sum_{a \in \cA} \left(\pi(h, s, a) \cdot \sum_{s' \in \cS} \trans_{|h| + 1}(s, a, s') \cdot \up^M(h + (s, a), s')\right).
    \end{align*}
    Putting this back into the above expression for $\mathrm{obj}(h, s)$, we get
    \begin{align*}
        & \phantom{\ = \ } \mathrm{obj}(h, s) \\
        & = z(h, s) \cdot \left(\sum_{a \in \cA} \vp_{|h| + 1}(s, a) \cdot \pi(h, s, a) + p(h, s)\right) \\
        & \phantom{\ = \ } + z(h, s) \cdot \sum_{a \in \cA} \left(\pi(h, s, a) \cdot \sum_{s' \in \cS} \trans_{|h| + 1}(s, a, s') \cdot \up^M(h + (s, a), s')\right) \\
        & = z(h, s) \cdot \left(\sum_{a \in \cA} \cdot \pi_{|h| + 1}(h, s, a) \cdot \left(\vp_{|h| + 1}(s, a) + \sum_{s' \in \cS} \trans_{|h| + 1}(s, a, s') \cdot \up^M(h + (s, a), s')\right) + p(h, s)\right) \\
        & = z(h, s) \cdot \up^M(h, s).
    \end{align*}
    So for any $h \in \cH$, $s \in \cS$, $\mathrm{obj}(h, s) = z(h, s) \cdot \up^M(h, s)$.
    Then we immediately have
    \begin{align*}
        \up^M(\emptyset) & = \sum_{s \in \cS} \trans_0(s) \cdot \up^M(\emptyset, s) = \sum_{s \in \cS} z(\emptyset, s) \cdot \up^M(\emptyset, s) = \sum_{s \in \cS} \mathrm{obj}(\emptyset, s) = \mathrm{obj}. \qedhere
        % & = \sum_{h \in \cH, s \in \cS: (h, s)\text{ is feasible}} \left(\sum_{a \in \cA} \vp_{|h| + 1}(s, a) \cdot x(h, s, a) + y(h, s)\right). \qedhere
    \end{align*}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ic1}]
    By Eq.~\eqref{eq:flow3} and Lemma~\ref{lem:util}, for all $h$, $s$, $s'$,
    \begin{align*}
        & \phantom{\ = \ } u(h, s, s') \\
        & = \sum_{a \in \cA} \va_{|h| + 1}(s, a) \cdot x(h, s', a) - y(h, s') \\
        & \phantom{\ =\ } + \sum_{a \in \cA, s'' \in \cS} \frac{\trans_{|h| + 1}(s, a, s'')}{\etrans_{|h| + 1}(s', a, s'')} \cdot z(h + (s', a), s'') \cdot \ua^M(h + (s', a), s'') \tag{Lemma~\ref{lem:util}} \\
        & = \sum_{a \in \cA} \va_{|h| + 1}(s, a) \cdot x(h, s', a) - y(h, s') + \sum_{a \in \cA, s'' \in \cS} \trans_{|h| + 1}(s, a, s'') \cdot x(h, s', a) \cdot \ua^M(h + (s', a), s'') \tag{Eq.~\eqref{eq:flow3}}
    \end{align*}
    Now by rearranging the above expression and applying the construction of the mechanism $M$ and the single-step reporting strategy $r_{h, s, s'}$, we have
    \begin{align*}
        & \phantom{\ = \ } u(h, s, s') \\
        & = \sum_{a \in \cA} x(h, s', a) \left(\va_{|h| + 1}(s, a) + \sum_{s'' \in \cS} \trans_{|h| + 1}(s, a, s'') \cdot \ua^M(h + (s', a), s'')\right) - y(h, s') \tag{rearranging} \\
        & = z(h, s') \cdot \left(\sum_{a} \pi(h, s', a) \cdot \left(\va_{|h| + 1}(s, a) + \sum_{s''} \trans_{|h| + 1}(s, a, s'') \cdot \ua^M(h + (s', a), s'')\right) - p(h, s')\right) \tag{construction of mechanism} \\
        & = z(h, s') \cdot \left(\sum_{a} \pi(h, s', a) \cdot \left(\va_{|h| + 1}(s, a) + \sum_{s''} \trans_{|h| + 1}(s, a, s'') \cdot \ua^{M, r_{h, s, s'}}(h + (s', a), s'')\right) - p(h, s')\right) \tag{construction of $r_{h, s, s'}$} \\
        & = z(h, s') \cdot \ua^{M, r_{h, s, s'}}(h, s), \tag{definition of $\ua^{M, r_{h, s, s'}}$}
    \end{align*}
    as desired.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ic2}]
    Fix $h \in \cH$, $s, s' \in \cS$, and let $(s_p, a_p) = \last(h)$.
    When $h = \emptyset$, by Lemmas~\ref{lem:util}~and~\ref{lem:ic1} and Eq.~\eqref{eq:flow2},
    \begin{align*}
        & \phantom{\ \iff \ } u(h, s) \ge \frac{\etrans_{|h|}(s_p, a_p, s)}{\etrans_{|h|}(s_p, a_p, s')} \cdot u(h, s, s') \\
        & \iff z(\emptyset, s) \cdot \ua^M(\emptyset, s) \ge \frac{\etrans_{0}(s_p, a_p, s)}{\etrans_{0}(s_p, a_p, s')} \cdot z(\emptyset, s') \cdot \ua^{M, r_{\emptyset, s, s'}}(\emptyset, s) \\
        & \iff z(\emptyset, s) \cdot \ua^M(\emptyset, s) \ge \frac{\etrans_{0}(s)}{\etrans_{0}(s')} \cdot z(\emptyset, s') \cdot \ua^{M, r_{\emptyset, s, s'}}(\emptyset, s) \\
        & \iff \ua^M(\emptyset, s) \ge \ua^{M, r_{\emptyset, s, s'}}(\emptyset, s).
    \end{align*}
    When $|h| > 0$, suppose $h = (s_1, a_1, \dots, s_t, a_t)$, and let $h_p = (s_1, a_1, \dots, s_{t - 1}, a_{t - 1})$.
    By Lemmas~\ref{lem:util}~and~\ref{lem:ic1} and Eq.~\eqref{eq:flow1},
    \begin{align*}
        & \phantom{\ \iff \ } u(h, s) \ge \frac{\etrans_{|h|}(s_p, a_p, s)}{\etrans_{|h|}(s_p, a_p, s')} \cdot u(h, s, s') \\
        & \iff z(h, s) \cdot \ua^M(h, s) \ge \frac{\etrans_{|h|}(s_p, a_p, s)}{\etrans_{|h|}(s_p, a_p, s')} \cdot z(h, s') \cdot \ua^{M, r_{h, s, s'}}(h, s) \\
        & \iff x(h_p, s_p, a_p) \cdot \ua^M(h, s) \ge x(h_p, s_p, a_p) \cdot \ua^{M, r_{h, s, s'}}(h, s).
    \end{align*}
    Note that when $x(h_p, s_p, a_p) = 0$, $(h, s)$ cannot be reached, because (1) if $z(h_p, s_p) > 0$, then when the (reported) history-state pair is $(h_p, s_p)$, the mechanism never takes action $a_p$, and (2) if $z(h_p, s_p) = 0$, then such an impossible action exists somewhere in $h_p$.
    In such cases, $\pi(h, s)$ and $p(h, s)$ will never be accessed, since it is impossible for the (reported) history to be $h$.
    In other words, when $(h, s)$ is reachable, we must have $x(h_p, s_p, a_p) > 0$, in which case the last inequality is equivalent to $\ua^M(h, s) \ge \ua^{M, r_{h, s, s'}}(h, s)$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ic}]
    We only need to show that IC is equivalent to robustness against single-step misreporting.
    We prove this inductively, aiming to eliminate misreporting one step at a time.
    To be more specific, consider the following partial reporting strategy.
    For a reporting strategy $r$, $t \in [T]$, let $r|_{\ge t}$ denote the reporting strategy restricted to time $t, t + 1, \dots, T$, i.e., for any $h' \in \cH$, $s' \in \cS$,
    \[
        r|_{\ge t}(h', s') = \begin{cases}
            s', \text{if } |h'| + 1 < t \\
            r(h', s'), \text{otherwise}
        \end{cases}.
    \]
    Similarly, let $r|_{< t}$ denote $r$ restricted to time $1, 2, \dots, t - 1$, and $r|_{= t}$ denote $r$ restricted to time $t$.
    We show inductively that for any reachable history-state pair $(h, s)$, and any reporting strategy $r$,
    \[
        \ua^{M, (r|_{< |h| + 1})}(h, s) \ge \ua^{M, r}(h, s).
    \]
    Without loss of generality, we assume that for any unreachable pair $(h', s')$, $r$ simply reports truthfully, i.e., $r(h', s') = s'$.

    Recall that $r(h)$ is the reported history given by $r$ when the true history is $h$.
    When $|h| = T - 1$, the above claim is implied by Lemma~\ref{lem:ic2}, because
    \[
        \ua^{M, r}(h, s) = \ua^{M, (r|_{\ge T})}(r(h), s) \ge \ua^M(r(h), s) = \ua^{M, (r|_{< T})}(h, s).
    \]
    Now suppose $|h| < T - 1$.
    By the induction hypothesis, we have
    \[
        \ua^{M, r}(h, s) = \ua^{M, (r|_{\ge |h| + 1})}(r(h), s) \le \ua^{M, ((r|_{\ge |h| + 1})|_{< |h| + 2})}(r(h), s) = \ua^{M, (r|_{= |h| + 1})}(r(h), s).
    \]
    Now again by Lemma~\ref{lem:ic2}, we have
    \[
        \ua^{M, r}(h, s) \le \ua^{M, (r|_{= |h| + 1})}(r(h), s) \le \ua^M(r(h), s) = \ua^{M, (r|_{< |h| + 1})}(h, s),
    \]
    which establishes the above claim.

    Now observe that as a special case of the claim, for any $s \in \cS$,
    \[
        \ua^{M, r}(\emptyset, s) \le \ua^{M, (r|_{< 1})}(\emptyset, s) = \ua^M(\emptyset, s).
    \]
    Now summing over $s$, this implies that for any reporting strategy $r$,
    \[
        \ua^{M, r}(\emptyset) = \sum_{s \in \cS} \trans_0(s) \cdot \ua^{M, r}(\emptyset, s) \le \sum_{s \in \cS} \trans_0(s) \cdot \ua^M(\emptyset, s) = \ua^M(\emptyset). \qedhere
    \]
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:short}]
    Given the correspondence between mechanisms and LP variables, by Lemma~\ref{lem:ic}, it is easy to see that (modulo the unreachable parts) every IC and IR mechanism corresponds bijectively to a feasible solution to the LP in Figure~\ref{fig:lp}.
    Moreover, by Lemma~\ref{lem:obj}, the objective value of this solution is precisely the principal's overall utility, which directly implies that an optimal solution to the LP corresponds to an IC and IR mechanism which maximizes the principal's overall utility.

    Now observe that the number of variables and the number of constraints in the LP are both $O(|\cS|^{T + 1} |\cA|^T)$.
    Moreover, all relevant coefficients in the LP can be encoded using $O(L)$ bits.
    It is well-known that such an LP can be solved in time $\mathrm{poly}(|\cS|^T, |\cA|^T, L)$.
\end{proof}


\section{Omitted Proofs from Section~\ref{sec:myopic}}

\begin{proof}[Proof of Lemma~\ref{lem:characterization}]
    We construct $M'$ explicitly based on $M$.
    Let $\pi'(t, s_p, a_p, s, a)$ be the probability that $M'$ chooses action $a$ at time $t$ in state $s$ when the previous state-action pair is $(s_p, a_p)$.
    Similarly, let $p'(t, s_p, a_p, s)$ be the payment specified by $M'$ at time $t$ in state $s$ when the previous state-action pair is $(s_p, a_p)$.
    We construct $M'$ from $M$ inductively as follows.
    \begin{comment}
    For each $s_p \in \cS$, $s_p \in \cS$ and $a_p \in \cA$, let $h^*(T, s_p, a_p)$ be any history such that
    \[
        h^*(T, s_p, a_p) \in \argmax_{h \in \cH_{T - 1}: (s_p, a_p) = \last(h)} \sum_{s \in \cS} \trans_{T - 1}(s_p, a_p, s) \cdot \left(\sum_{a \in \cA} \pi(h, s, a) \cdot \vp_{|T|}(s, a) + p(h, s)\right),
    \]
    and for all $s \in \cS$, let
    \[
        \pi'(T, s_p, a_p, s) = \pi(h^*(T, s_p, a_p), s) \quad \text{and} \quad p(T, s_p, a_p, s) = p(h^*(T, s_p, a_p), s).
    \]
    Then, for each $t \in [T - 1]$, $s_p \in \cS$ and $a_p \in \cA$, let $h^*(t, s_p, a_p)$ be any history such that
    \begin{align*}
        h^*(t, s_p, a_p) \in \argmax_{h \in \cH_{t - 1}: (s_p, a_p) = \last(h)} \sum_{s \in \cS} \trans_{t - 1}(s_p, a_p, s) \cdot & \left(p(h, s) + \sum_{a \in \cA} \pi(h, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} \right. \right. \\
        & \left. \left. + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^{M'}(h + (s, a), s')\right)\right).
    \end{align*}
    Note that the above $h^*(t, s_p, a_p)$ is well-defined, in particular because $\up^{M'}(h + (s, a), s')$ depends only on $\pi'(t', s_p', a_p', s)$ and $p'(t', s_p', a_p', s)$ for $t' > t$, and not on any part of $M'$ that is not yet constructed.
    Then similarly, for all $s \in \cS$, let
    \[
        \pi'(t, s_p, a_p, s) = \pi(h^*(t, s_p, a_p), s) \quad \text{and} \quad p(t, s_p, a_p, s) = p(h^*(t, s_p, a_p), s).
    \]
    \end{comment}
    For each $t \in [T]$, $s_p \in \cS$ and $a_p \in \cA$, let $h^*(t, s_p, a_p) \in \cH_{t - 1}$ be any history such that
    \begin{align*}
        h^*(t, s_p, a_p) \in \argmax_{h \in \cH_{t - 1}: (s_p, a_p) = \last(h)} \sum_{s \in \cS} \trans_{t - 1}(s_p, a_p, s) \cdot & \left(p(h, s) + \sum_{a \in \cA} \pi(h, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} \right. \right. \\
        & \left. \left. + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^M(h + (s, a), s')\right)\right).
    \end{align*}
    Then, for all $s \in \cS$, let
    \[
        \pi'(t, s_p, a_p, s) = \pi(h^*(t, s_p, a_p), s) \quad \text{and} \quad p(t, s_p, a_p, s) = p(h^*(t, s_p, a_p), s).
    \]
    This finishes the construction of $M'$.

    We first show that $\up^{M'}(\emptyset) \ge \up^M(\emptyset)$, by inductively showing a stronger claim: for all $h \in \cH$,
    \[
        \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \up^{M'}(h, s) \ge \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \up^M(h, s),
    \]
    where $(s_p, a_p) = \last(h)$.
    For all $h \in \cH_{T - 1}$, letting $(s_p, a_p) = \last(h)$, by the construction of $M'$, we have
    \begin{align*}
        \sum_s \trans_{T - 1}(s_p, a_p, s) \cdot \up^{M'}(h, s) & = \sum_s \trans_{T - 1}(s_p, a_p, s) \cdot \up^M(h^*(T, s_p, a_p), s) \\
        & \ge \sum_s \trans_{T - 1}(s_p, a_p, s) \cdot \up^M(h, s).
    \end{align*}
    Now for all $h \in \cH$ where $|h| < T - 1$, letting $(s_p, a_p) = \last(h)$ and $h^* = h^*(|h| + 1, s_p, a_p)$, we have
    \begin{align*}
        & \phantom{\ =\ } \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \up^{M'}(h, s) \\
        & = \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \left(p(h^*, s) + \sum_{a \in \cA} \pi(h^*, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^{M'}(h + (s, a), s')\right)\right) \\
        & = \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \left(p(h^*, s) + \sum_{a \in \cA} \pi(h^*, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^{M'}(h^* + (s, a), s')\right)\right) \tag{property of $M'$} \\
        & \ge \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \left(p(h^*, s) + \sum_{a \in \cA} \pi(h^*, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^M(h^* + (s, a), s')\right)\right) \tag{induction hypothesis} \\
        & \ge \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \left(p(h, s) + \sum_{a \in \cA} \pi(h, s, a) \cdot \left(\vp_{|h| + 1}(s, a) \vphantom{\sum_{s' \in \cS}} + \sum_{s' \in \cS} \trans_t(s, a, s') \cdot \up^M(h + (s, a), s')\right)\right) \tag{choice of $h^*$} \\
        & = \sum_s \trans_{|h|}(s_p, a_p, s) \cdot \up^M(h, s).
    \end{align*}
    Then in particular, we have
    \[
        \up^{M'}(\emptyset) = \sum_s \trans_0(s) \cdot \up^{M'}(\emptyset, s) \ge \sum_s \trans_0(s) \cdot \up^M(\emptyset, s) = \up^M(\emptyset).
    \]

    Finally we prove that $M'$ is IC.
    By the proof of Lemma~\ref{lem:ic}, we only need to show that $M'$ is robust against any single-step reporting strategy $r_{h, s, s'}$.
    In fact, letting $(s_p, a_p) = \last(h)$ and $h^* = h^*(|h| + 1, s_p, a_p)$,
    \[
        \ua^{M'}(h, s) = \sum_a \pi(h^*, s, a) \cdot \va_{|h| + 1}(s, a) + p(h^*, s) = \ua^M(h^*, s).
    \]
    Moreover,
    \[
        \ua^{M', r_{h, s, s'}}(h, s) = \sum_a \pi(h^*, s', a) \cdot \va_{|h| + 1}(s, a) + p(h^*, s) = \ua^{M, r_{h, s, s'}}(h^*, s).
    \]
    Since $M$ is IC, we have
    \[
        \ua^{M'}(h, s) = \ua^M(h^*, s) \ge \ua^{M, r_{h, s, s'}}(h^*, s) = \ua^{M', r_{h, s, s'}}(h, s).
    \]
    Now by the argument in the proof of Lemma~\ref{lem:ic}, we know that for all reporting strategy $r$, $h \in \cH$, $s \in \cS$,
    \[
        \ua^{M', r}(h, s) \le \ua^{M', (r|_{< |h| + 1})}(h, s),
    \]
    so
    \[
        \ua^{M', (r|_{\ge |h| + 1})}(h, s) \le \ua^{M', ((r|_{\ge |h| + 1})|_{< |h| + 1})}(h, s) = \ua^{M'}(h, s),
    \]
    which is precisely the IC requirement for myopic agents.
    Similar arguments guarantee that $M'$ has the same IR property as $M$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:myopic}]
    We first argue the easy part, i.e., the time complexity.
    Observe that calls to $\optstatmech$ dominates the time complexity.
    Moreover, the algorithm makes $T |\cS| |\cA|$ calls to $\optstatmech$, so the overall time complexity is as stated.

    Now we show the optimality of the computed mechanism $M$.
    We prove inductively a stronger claim, i.e., for any $t \in [T]$, $s_p \in \cS$, $a_p \in \cA$,
    \[
        \sum_s \trans_0(s_p, a_p, s) \cdot \up^M(t, s_p, a_p, s) = \max_{M'} \trans_0(s_p, a_p, s) \cdot \up^{M'}(t, s_p, a_p, s),
    \]
    where the maximum is over all succinct mechanisms $M'$ that are IC and (optionally) IR.
    First observe that for all $s \in \cS$, $a \in \cA$,
    \[
        u(T, s, a) = \vp_T(s, a).
    \]
    So, for all $s_p \in \cS$, $a_p \in \cA$,
    \begin{align*}
        & \phantom{\ =\ } \sum_s \trans_0(s_p, a_p, s) \cdot \up^M(T, s_p, a_p, s) \\
        & = \sum_s \trans_0(s_p, a_p, s) \cdot \left(p(T, s_p, a_p, s) + \sum_a \pi(T, s_p, a_p, s, a) \cdot \vp_T(s, a)\right) \\
        & = \max_{M' = (\pi', p')} \sum_s \trans_0(s_p, a_p, s) \cdot \left(p'(T, s_p, a_p, s) + \sum_a \pi'(T, s_p, a_p, s, a) \cdot \vp_T(s, a)\right) \tag{optimality of $M$ at time $T$ as a static mechanism} \\
        & = \max_{M'} \sum_s \trans_0(s_p, a_p, s) \cdot \up^M(T, s_p, a_p, s).
    \end{align*}
    Again, the maximum is over all succinct mechanisms $M'$ that are IC and (optionally) IR.

    Now for $t \in [T - 1]$, by the construction of $M$,
    \begin{align*}
        & \phantom{\ =\ } \sum_s \trans_0(s_p, a_p, s) \cdot \up^M(t, s_p, a_p, s) \\
        & = \sum_s \trans_0(s_p, a_p, s) \cdot \left(p(t, s_p, a_p, s) + \sum_a \pi(t, s_p, a_p, s, a) \cdot \left(\vp_t(s, a) \vphantom{\sum_{s'}} \right.\right. \\
        & \phantom{\ =\ } \left.\left. + \sum_{s'} \trans_t(s, a, s') \cdot \up^M(t + 1, s, a, s')\right)\right) \\
        & = \max_{M' = (\pi', p')} \sum_s \trans_0(s_p, a_p, s) \cdot \left(p'(t, s_p, a_p, s) + \sum_a \pi'(t, s_p, a_p, s, a) \cdot \left(\vp_t(s, a) \vphantom{\sum_{s'}} \right.\right. \\
        & \phantom{\ =\ } \left.\left. + \sum_{s'} \trans_t(s, a, s') \cdot \up^M(t + 1, s, a, s')\right)\right). \tag{optimality of $M$ at time $t$ as a static mechanism}
    \end{align*}
    By the induction hypothesis and the fact that $M'$ is succinct,
    \begin{align*}
        & \phantom{\ =\ } \sum_s \trans_0(s_p, a_p, s) \cdot \up^M(t, s_p, a_p, s) \\
        & = \max_{M' = (\pi', p')} \sum_s \trans_0(s_p, a_p, s) \cdot \left(p'(t, s_p, a_p, s) + \sum_a \pi'(t, s_p, a_p, s, a) \cdot \left(\vp_t(s, a) \vphantom{\sum_{s'}} \right.\right. \\
        & \phantom{\ =\ } \left.\left. + \max_{M''} \sum_{s'} \trans_t(s, a, s') \cdot \up^{M''}(t + 1, s, a, s')\right)\right) \tag{induction hypothesis} \\
        & = \max_{M' = (\pi', p')} \sum_s \trans_0(s_p, a_p, s) \cdot \left(p'(t, s_p, a_p, s) + \sum_a \pi'(t, s_p, a_p, s, a) \cdot \left(\vp_t(s, a) \vphantom{\sum_{s'}} \right.\right. \\
        & \phantom{\ =\ } \left.\left. + \sum_{s'} \trans_t(s, a, s') \cdot \up^{M'}(t + 1, s, a, s')\right)\right) \tag{$M'$ is succinct} \\
        & = \max_{M'} \sum_s \trans_0(s_p, a_p, s) \cdot \up^{M'}(t, s_p, a_p, s).
    \end{align*}
    All maxima are over all succinct mechanisms that are IC and (optionally) IR.
    As a result, we have
    \[
        \up^M(\emptyset) = \sum_s \trans_0(s) \cdot \up^M(\emptyset, s) = \max_{M'} \sum_s \trans_0(s) \cdot \up^{M'}(\emptyset, s) = \max_{M'} \up^{M'}(\emptyset). \qedhere
    \]
\end{proof}


\section{Omitted Proofs from Section~\ref{sec:memoryless}}

\begin{proof}[Proof of Theorem~\ref{thm:suboptimality}]
    First suppose the agent is patient and without loss of generality has a discount factor of $1$.
    Let $T = 2$ and $\cS = \cA = [n]$ where $n \ge \eps^{-1}$.
    The initial distribution is uniform over $[n]$, i.e., $\trans_0(i) = 1 / n$ for all $i \in [n]$, i.e., no matter what action is played, all states always transition to state $1$.
    The transition operator is such that $\trans_1(i, j, 1) = 1$ for all $i, j \in [n]$.
    At time $T = 2$, the principal's valuations are $\vp_T(i, j) = 0$ for all $i, j \in [n]$.
    At time $1$, the principal's valuation function is such that for all $i, j \in [n]$, $\vp_1(i, j) = 1$ if $i = j$, and $\vp_1(i, j) = 0$ if $i \ne j$.
    For $t \in [T]$, the agent's valuation function is such that for all $i, j \in [n]$, $\va_t(i, j) = 0$ if $i = j$, and $\va_t(i, j) = 1$ if $i \ne j$.

    Consider the principal's optimal utility, which is clearly upper bounded by $1$ ($1$ at time $1$ and $0$ at time $2$).
    The following mechanism is IC and achieves this upper bound:
    \begin{itemize}
        \item At time $1$, play action $i$ for each state $i \in [n]$.
        \item At time $T = 2$, play action $(i \bmod n) + 1$ iff the state at time $1$ is $i$.
    \end{itemize}
    The mechanism is IC because regardless of the (reported) initial state, the agent achieves overall utility $1$.
    It is easy to check this mechanism achieves utility $1$.

    On the other hand, any memoryless IC mechanism can achieve utility at most $1 / n \le \eps$.
    This is because at time $T = 2$, the current state provides absolutely no information, so the mechanism has to perform the same (randomized) action regardless of the initial state.
    As a result, in order to be IC, the mechanism has to satisfy the following condition at time $1$: for all $i, j \in [n]$, $\pi(i, i) \le \pi(j, i)$, where $\pi(a, b)$ is the probability that action $b$ is played in state $a$ at time $1$.
    So the principal's utility can be bounded as follows:
    \[
        \frac1n \sum_i \pi(i, i) \le \frac1n \sum_i \left(\frac1n \sum_j \pi(j, i)\right) = \frac{1}{n^2} \sum_{i, j} \pi(j, i) = \frac1n.
    \]
    This concludes the proof when the agent is patient.

    Now consider the case with a myopic agent.
    Again, let $T = 2$ and $\cS = \cA = [n]$ where $n \ge \eps^{-1}$.
    The initial distribution is again uniform over $[n]$, i.e., $\trans_0(i) = 1 / n$ for all $i \in [n]$.
    The transition operator is such that $\trans_1(i, j, i) = 1$ for all $i, j \in [n]$, i.e., no matter what action is played, state $i$ always transitions to state $i$.
    At time $1$, the principal's and the agent's valuations are $\vp_1(i, j) = \va_1(i, j) = 0$ for all $i, j \in [n]$.
    At time $T = 2$, the principal's valuation function is such that for all $i, j \in [n]$, $\vp_T(i, j) = 1$ if $i = j$, and $\vp_T(i, j) = 0$ if $i \ne j$.
    And the agent's valuation function is such that for all $i, j \in [n]$, $\va_T(i, j) = 0$ if $i = j$, and $\va_T(i, j) = 1$ if $i \ne j$.

    The principal's optimal utility, $1$, is achieved by the following succinct (but not memoryless) IC mechanism:
    \begin{itemize}
        \item At time $1$, play action $1$ for all states.
        \item At time $2$, play action $i$ iff the state at time $1$ is $i$.
    \end{itemize}
    The mechanism is IC in particular because the agent is myopic and cannot change the past.
    It is easy to check this mechanism achieves utility $1$.

    On the other hand, any memoryless IC mechanism can achieve utility at most $1 / n \le \eps$.
    This is because at time $T = 2$, the mechanism cannot memorize anything before, so it has to be IC based only on the current state, which puts the mechanism in a situation that is essentially the same as at time $1$ in the hard instance for patient agents.
    Similar arguments then guarantee that the principal's utility is at most $1 / n$, which concludes the proof for myopic agents.
    Finally, we note that the above constructions work even if payments are allowed.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:np-hardness}]
    We use reductions from MAX-SAT similar to that in Theorem~\ref{thm:long} for both myopic and patient agents.
    First consider the case where the agent is patient with a discount factor of $1$.
    In this case, the reduction in Theorem~\ref{thm:long} applies without any modification.
    In particular, since the principal and the agent are in a zero-sum situation, without loss of generality, any optimal memoryless mechanism does not depend on the reported states.
    And again, since the principal's utility is multilinear in the actions at each time, there is a deterministic mechanism which is optimal.
    As argued in the proof of Theorem~\ref{thm:long}, such a mechanism corresponds precisely to an optimal assignment of variables in the MAX-SAT instance, which implies the $7/8 + \eps$ inapproximability.

    Now consider the case where the agent is myopic.
    Here we slightly modify the reduction, and in particular, the agent's valuation functions.
    That is, for each $t \in [T]$ and $i \in [m]$, we let
    \[
        \va_t(s, a_\mathrm{pos}) = c \quad \text{and} \quad \va_t(s, a_\mathrm{neg}) = 0,
    \]
    for all $s \in \cS$, where $c > 0$ is an arbitrarily small constant.
    This guarantees that at any time $t$, in order to be IC, the (randomized) actions for all states have to be exactly the same.
    Then since the principal's utility is multilinear, again it is without loss of generality to consider deterministic mechanisms, which correspond to assignments of variables.
    The ratio of $7/8 + \eps$ follows immediately.
    Finally, we remark that the above reductions still work when payments are allowed.
\end{proof}
